Improved Deep Point Cloud Geometry Compression

Point clouds have been recognized as a crucial data structure for 3D content and are essential in a number of applications such as virtual and mixed reality, autonomous driving, cultural heritage, etc. In this paper, we propose a set of contributions to improve deep point cloud compression, i.e.: using a scale hyperprior model for entropy coding; employing deeper transforms; a different balancing weight in the focal loss; optimal thresholding for decoding; and sequential model training. In addition, we present an extensive ablation study on the impact of each of these factors, in order to provide a better understanding about why they improve RD performance. An optimal combination of the proposed improvements achieves BD-PSNR gains over G-PCC trisoup and octree of 5.50 (6.48) dB and 6.84 (5.95) dB, respectively, when using the point-to-point (point-to-plane) metric. Code is available at https://github.com/mauriceqch/pcc_geo_cnn_v2 .

==> fig_soldier_c4ws_tris_hbr_errors.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/soldier_c4ws_tris_hbr/errors.hist.pdf}
    \caption{Histogram of D1 squared errors for \condsequential{} and G-PCC Trisoup.}
\end{figure}
